Winning the Caucus Race: Continuous Leader Election via Public Randomness

Consensus protocols inherently rely on the notion of leader election, in which one or a subset of participants are temporarily elected to authorize and announce the network's latest state. While leader election is a well studied problem, the rise of distributed ledgers (i.e., blockchains) has led to a new perspective on how to perform large-scale leader elections via solving a computationally difficult puzzle (i.e., proof of work). In this paper, we present Caucus, a large-scale leader election protocol with minimal coordination costs that does not require the computational cost of proof-of-work. We evaluate Caucus in terms of its security, using a new model for blockchain-focused leader election, before testing an implementation of Caucus on an Ethereum private network. Our experiments highlight that one variant of Caucus costs only $0.10 per leader election if deployed on Ethereum.

==> beacon.tex <==
\section{Shared Randomness}\label{sec:beacon}
As explained in Section~\ref{sec:randao}, we are interested in secure collective
coin flipping protocols to initialize our beacon $\globalrandao$. In this section we present
two protocols that achieve this goal.
In
the literature, most of these types of \emph{random beacons} are based on
secret sharing protocols (see Appendix~\ref{appendix:scrape} for definitions
of secret sharing).  The ones that are most appropriate for our setting are
RandHound~\cite{randhound}, and
SCRAPE~\cite{scrape}, so to explain our choices we briefly examine each of
them in turn.
\saraha{should I add randshare?}

% \subsection{Randshare}
% Randhsare~\cite{randhound} is a collective coin tossing protocol that ensure liveness,
% unbiasability and unpredictability.


%random beacons -> coin tossing property for each round
%cite Joe's paper and Rabin transaction protection by beacons

% A comparison of these protocols, as well as the three protocols
% we already described, is in Table~\ref{tab:coordination}.

% \begin{table*}
% \centering
% \begin{tabular}{lccccc}
% \toprule
%  & \# phases & \#messages\\%coordination \\%& \# blocks \\%& \#messages\\
% \midrule
% Snow White  & 1 & $O(n)$ \\% 1 transaction/& 2$\omega$ + &\\
% Ouroboros  & 3 &  $O(nc)$ \\%n+2t transactions (best case: 2n transactions)/& 10k slots \\
% Algorand & 1 & $O(n)$\\
% %Algorand  & m  & \# of steps * \#verifiers &  \\
% %Threshold relay  &  & 0 & 0 & $(group size)^2$\\
% \midrule
% RandHound  & 7 &  $O(nc^2)$   & \\
% Scrape & 3& $O(n^2)$ \\%n+2t transactions (best case: 2n transactions)
% % private randomness  & 0 & 0 & 0 &0\\
% % mauve  & 1 &0 & 0&0\\
% % hybrid randomness & 3 & n & 0 & 0\\
% \bottomrule
% \end{tabular}
% \caption{Comparison of coordination for random beacons.  For Ouroboros, $c$
% is the size of the randomly selected committee.  For RandHound,
% $c$ is the size of the shard.}
% \label{tab:coordination}
% \end{table*}

% \subsubsection{Ouroboros}
%
% Briefly, each member $P_i$ of the subcommittee
% randomly generates a secret $s^i$ and then computes shares $(s_1^i,\dots,
% s_n^i)$ of this secret, where each share $s_j^i$ is encrypted using the public
% key of participant $j$.  They then embed their list of encrypted shares,
% together with a commitment to each shares, on the blockchain.
% Upon decrypting their shares, participants verify whether they were correctly computed
% using the commitments. They then start a Byzantine agreement for every secret.
% If the share for secret $s_j^i$ was computed correctly, participant $P_j$ broadcast a positive vote for this share. If they receive enough positive votes for secret $s^i
% $ from other participants,
% they send a positive commit for this value. If $2f+1$ positive commits are received for
% a value, participants consider this value for the final randomness, else they don't.
% After a decision has been made for every value, participants embed an opening to their
% commitment on the blockchain, thus revealing their secret $s^i$.  If a
% participant $P_i$ doesn't open their commitment, then after some additional
% number of blocks, other participants reveal their decrypted shares, $s_j^i$,
% of the missing values.  This allows them to recover commitments that haven't
% been opened, as long as there are enough honest participants.  The random
% value is then taken to be the XOR of all the $s_i$ values.
%
% While this protocol satisfies liveness and unpredictability, participants do
% not verify the encrypted shares at the time they are
% first placed on the blockchain (i.e., do not verify that the value in the
% commitment and the cumulative value in the encrypted shares are the same).
% This means that an adversary could compute bad shares and thus bias the
% protocol by opening the commitment if it works in their favor, or forcing the
% other participants to recover the secret if not.

\subsection{RandHound}

RandHound~\cite{randhound} uses publicly verifiable secret sharing.
%, which
%solves the issue presented by Ouroboros.
% Similarly to the idea of a
% subcommittee,
It uses \emph{shards}, where peers share their secrets
only within their smaller group, to improve scalability.

In RandHound, a client interacts with a network of servers in order to obtain
a publicly verifiable random number.
In the initialization phase, the client randomly creates balanced grouping of the servers.
Participants then create shares of their
secret only for the members of their group, and send their encrypted
shares to the client together with a non-interactive zero-knowledge proof
(NIZK) that the shares are computed correctly.  The client then chooses a set
of inputs from each group that provided valid shares.  This allows
the protocol to achieve liveness, since even if a server provided invalid
shares, their input will not count toward the final result
and the protocol can continue.
The servers acknowledge the client's choice of inputs by collectively signing it.
After the client obtains the signature on their
choice of inputs, they can request servers to decommit to their secret.
The client then combine all the shares to form the final randomness. \sarahm{This is much more informal than
the description of Ouroboros, and a bit confusing in places.}
Randhound optimize on scalability by using smaller groups, this does not
really fit the context of blockchains where transactions (and thus all messages)
are broadcast to the whole network. We next present SCRAPE, a publicly verifiable
randomness generation algorithm that was designed in the context of distributed ledgers.
\sarahm{Should end as we did with Ouroboros by saying why we don't plan to use
this.  Is it because it considers explicit coordination rather than
blockchains?}

\subsection{SCRAPE}
SCRAPE~\cite{scrape} propose a verifiable secret sharing scheme that requires a linear number of exponentiation for sharing, verification and reconstruction.
%The idea is similar to the coin-tossing used in Ouroboros.
Briefly, each member $P_i$
randomly generates a secret $s_i$ and then computes shares $(s_1^i,\dots,
s_n^i)$ of this secret, where each share $s_j^i$ is encrypted using the public
key of participant $j$.  They then embed their list of encrypted shares,
together with a commitment to their secret, on the blockchain.
Participants also embed a proof that these shares were correctly computed.
Given the encrypted shares, together with the proof, every participants can verify
that the shares are computed correctly and
only valid shares are considered for the final random number.
After this commit phase, participants embed an opening to their
commitment on the blockchain, thus revealing their secret $s_i$.  If a
participant $P_i$ doesn't open their commitment, then other participants reveal
their decrypted shares, $s_j^i$,
of the missing values.  This allows them to recover commitments that haven't
been opened, as long as there are enough honest participants.
%Participants create shares of their
%randomly generated secret $s_i$ and encrypt these shares with other participants' public key
%and publish these to the blockchain together with a commitment to their secret.
% The difference here is that participants also embeds a proof that these shares were correctly computed.
% Given the encrypted shares, together with the proof, every participants can verify
% that the shares are computed correctly and
% only valid shares are considered for the final random number.
% Then similarly to~\cite{iohk-pos}, participants open their commitments, if they do not,
% other participants post their decrypted shares for that secret on the blockchain, allowing
% the remaining participants to recover the secret.
The output of the protocol is then taken as a combination of the secrets.

Based on the previous comparison, we decided to use SCRAPE for our instantiation.
However this solution still requires an important amount of coordination.
We give a more detailed description of SCRAPE in Appendix~\ref{appendix:scrape}.
Moreover we highlight that this protocol is similar to the one used for generating
randomness in the Ouroboros proof-of-stake protocol~\cite{iohk-pos} (although they use a different
PVSS scheme).

%\begin{table*}
%\centering
%\begin{tabular}{lcccc}
%\toprule
%& unbiasable & unpredictable & liveness  \\
%\midrule
%Snow White & not really & not really & yes  \\
%%Snow white adaptation & yes & no & no \\
%Ouroboros & yes & yes & yes  \\
%Algorand & yes & yes & yes  \\
%RandHound & yes & yes & yes  \\
%%Threshold relay & yes & yes  & no  \\
%% \midrule
%% private randomness & yes & no & yes \\
%% mauve & yes & kind of & no \\
%% hybrid randomness & yes & yes & yes \\
%Scrape & yes & yes & yes \\
%\bottomrule
%\end{tabular}
%\end{table*}


==> pvss.tex <==
%\section{(Publicly Verifiable) Secret Sharing}\label{sec:defns-vss}
%
%A $(n,t)$-threshold secret sharing scheme~\cite{shamir79} consists of a set of $n$
%participants $(P_1,\dots,P_n)$ and a dealer $\dealer$ who distributes shares
%$(s_1,\ldots,s_n)$ of a secret $s$ among the participants in such a way that
%$t$ or more of them can recover the secret $s$.
%
%A publicly verifiable secret sharing (PVSS)
%scheme~\cite{FOCS:CGMA85,C:Schoenmakers99} has the additional property
%that anyone can verify that the shares have been computed correctly and allow
%the participants to recover a valid secret. In such
%a scheme, the dealer publishes encrypted versions of the shares $(\hat{s}_1,
%\dots,\hat{s}_n)$, where each share is encrypted with the public key $\pk_i$
%of one of the participants, along with a proof $\pi_\dealer$ that these
%ciphertexts correspond to valid shares of some secret.  Anyone with access to
%the encrypted shares can then verify this proof.  Later, when a participant
%$P_i$ decrypts their share $\hat{s}_i$, they publish a proof $\pi_i$
%of a valid decryption, that again anyone with access to the decrypted share
%should be able to verify.
%
%Informally, the security properties that such a scheme must satisfy are~\cite{scrape}:
%(1) correctness: if the dealer and participants are honest then the secret can be recovered
%with $t$ shares and all verification must verify; (2) verifiability: if the verification
%passes then, with high probability, the shares are correctly computed, i.e. they allow
%the paticipants to recover the secret $s$; (3) IND1-secrecy: the encrypted shares, together with
%$t-1$ secret keys $\{\sk_i\}$ do not give any information about the secret.

